Quenched $B_K$-parameter from Osterwalder-Seiler tmQCD quarks and mass-splitting discretization effects

We apply an Osterwalder-Seiler version of twisted mass QCD to a study of the $B_K$ parameter, in which three of the four quark fields making up the relevant $\Delta S =2$ operator are maximally twisted with the same twist angle, while the fourth one has a twist angle of opposite sign. It is known that this setup ensures automatic improvement of the bare $K^0$-$\overline K^0$ operator matrix element and multiplicative renormalization of the $\Delta S =2$ operator, at the price of breaking the $K^0$-$\overline K^0$ mass degeneracy by discretization effects. As a result, two dominant systematic errors of the $B_ K$ determination with Wilson fermions are kept under control. With the Clover term included in the fermion action, we perform a feasibility study and find, in the quenched approximation, a significant improvement of the scaling behaviour of $B_K$, compared to earlier standard tmQCD determinations. Moreover, we study in detail the $K^0$-$\overline K^0$ mass splitting that characterizes this approach and confirm that, in the presence of the Clover term, it is greatly reduced in a maximally twisted theory.

==> diff <==
4,5c4,12
< In this work we have addressed a couple of issues related to the proposal of ref.~\cite{Frezzotti:2004wz} for the computation of $B_{\rm K}$ in a tmQCD setup, using a four-fermion operator made of two tm-type
< quarks and two OS-type quarks, all maximally twisted. This ensures that the operator is multiplicatively renormalizable and automatically improved. The price to pay is that in this way the Kaon and anti-Kaon states of the weak matrix element $\langle \overline K^0 | O^{\Delta S = 2} | K^0 \rangle$ are composed of different lattice quark field combinations (tm and OS) and thus are non degenerate at finite lattice spacing.
---
> In this work we have addressed a couple of issues related to the proposal 
> of ref.~\cite{Frezzotti:2004wz} for the computation of $B_{\rm K}$ in a 
> tmQCD setup, using a four-fermion operator made of two tm-type
> quarks and two OS-type quarks, all maximally twisted. This ensures that 
> the operator is multiplicatively renormalizable and automatically improved. 
> The price to pay is that in this way the Kaon and anti-Kaon states of the 
> weak matrix element $\langle \overline K^0 | O^{\Delta S = 2} | K^0 \rangle$ 
> are composed of different lattice quark field combinations (tm and OS) and 
> thus are non degenerate at finite lattice spacing.
7c14,27
< We have performed a quenched study in order to address these issues. In particular, we find that the inclusion of the Clover term in the fermionic action significantly reduces the mass splitting between Kaon and anti-Kaon at finite lattice spacing. This result, already observed in an earlier work at a single lattice spacing, has been confirmed by us for several $\beta$-values. It should also be noted that in earlier studies, in which a Clover term was not included in the action,  this mass splitting, besides being much bigger than the one we measure, was found to be significantly affected by the choice of non-perturbative procedure for tuning the lattice theory to maximal twist. This does not appear to be the case once an $O(a)$ Symanzik-improved procedure, with a standard (untwisted) mass term, is used to tune the hopping parameter to its critical value. We also confirm that this splitting decreases as the continuum limit is approached.
---
> We have performed a quenched study in order to address these issues. 
> In particular, we find that the inclusion of the Clover term in the 
> fermionic action significantly reduces the mass splitting between 
> Kaon and anti-Kaon at finite lattice spacing. This result, already 
> observed in an earlier work at a single lattice spacing, has been 
> confirmed by us for several $\beta$-values. It should also be noted 
> that in earlier studies, in which a Clover term was not included in 
> the action,  this mass splitting, besides being much bigger than the 
> one we measure, was found to be significantly affected by the choice 
> of non-perturbative procedure for tuning the lattice theory to maximal 
> twist. This does not appear to be the case once an $O(a)$ Symanzik-improved 
> procedure, with a standard (untwisted) mass term, is used to tune the 
> hopping parameter to its critical value. We also confirm that this 
> splitting decreases as the continuum limit is approached.
9c29,36
< The second objective of the present paper is the presentation of first results for $B_{\rm K}$, obtained in this tm-OS setup. We have compared our results to the earlier ones of refs.~\cite{Dimopoulos:2006dm,Dimopoulos:2007cn}, in which $B_{\rm K}$ had been computed in a tmQCD setup, without maximal twist on all flavours and thus without automatic $O(a)$-improvement. These results were rather sensitive to discretization errors, as revealed by the dependence of $B_{\rm K}$ on the Symanzik $O(a)$ term of the axial current at coarser lattice spacings.
---
> The second objective of the present paper is the presentation of first 
> results for $B_{\rm K}$, obtained in this tm-OS setup. We have compared 
> our results to the earlier ones of refs.~\cite{Dimopoulos:2006dm,Dimopoulos:2007cn}, 
> in which $B_{\rm K}$ had been computed in a tmQCD setup, without maximal 
> twist on all flavours and thus without automatic $O(a)$-improvement. 
> These results were rather sensitive to discretization errors, as revealed 
> by the dependence of $B_{\rm K}$ on the Symanzik $O(a)$ term of the axial 
> current at coarser lattice spacings. 
11c38
< $O(a)$-improved, leaving us only with $O(a\Lambda_{\rm QCD})$ effects from
---
> $O(a)$-improved, leaving us only with $O(a\Lambda_{\rm QCD}$ effects from
13c40
< display significantly better scaling, compatible with  an $O(a^2)$
---
> display significantly better scaling, compatible with an $O(a^2)$
15d41
< 


==> paper_parts/acknow.tex <==
\section*{Acknowledgments}
We gratefully acknowledge the participation of F.~Palombi at the early stages of this work and thank him for his help and suggestions. We also wish to thank R.~Frezzotti, G.~Herdoiza, C.~Pena, S.~Sint and G.C.~Rossi for discussions. We thank INFN-``Tor Vergata" and Milano-Bicocca for providing hospitality to members of our collaboration at various stages of this work and the DESY-Zeuthen computing centre for its support. This work was supported in part by the EU Contract No. MRTN-CT-2006-035482, "FLAVIAnet".

==> paper_parts/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this work we have completed our study of basic kaon weak matrix elements
in quenched Wilson tmQCD.
Our final value for $F_K$ is the best controlled quenched result obtained 
with Wilson fermions from the point of view of systematic uncertainties. 
We have also provided a final value for $B_K$, with an error that, in 
our view, reflects faithfully the best accuracy that can be expected 
for this quantity in the absence of full $\Oa$ improvement.
Finally, we have performed a thorough study of flavour breaking in
our version of tmQCD, confirming that it does not introduce
any uncontrolled systematics in our results.
\parbreak
The dominant source of uncertainty left in the quenched approximation
(certainly so for $B_K$) is related to the lack of full $\Oa$ improvement, which
amplifies the error of the continuum limit extrapolation. Thus, if Wilson
fermions are to be used in the future in the determination of weak matrix
elements, the use of tmQCD variants that embody automatic $\Oa$ improvement
\cite{Frezzotti:2004wz} may prove essential. Two important aspects of the tmQCD
approach are crucial in the context of weak matrix elements: the tuning of
mass parameters, in particular of the twist angle, has to be controlled to high
precision; and flavour symmetry breaking effects should be reasonably small, 
as in the present study. In conclusion, the present work
demonstrates that, once the tuning of the twisted angle and flavour symmetry
breaking are under control, tmQCD may offer a convenient alternative to other 
discretizations. As we are entering the era of tmQCD simulations with 
dynamical quarks \cite{Boucaud:2007uk}, it will be important to explore 
these issues in future unquenched studies. 
 


==> paper_parts/intro.tex <==
\section{Introduction}
\label{sec:intro}

The bag parameter of neutral $K$-meson oscillations $B_{\rm K}$, has been the object of many lattice QCD computations. Several discretizations of lattice fermions have been implemented for this purpose. The most recent quenched result~\cite{Nakamura:2008xz} has reached a precision of about $1\%$. Attention has now shifted to unquenched estimates; see REF for a recent review. 

The Wilson fermion results of $B_K$ are normally the least accurate, due to a limited control of two sources of systematic error:
\begin{enumerate}
\item
Loss of chiral symmetry causes the relevant $\Delta S = 2$ four-fermion operator to mix, under renormalization, with four other operators of the same dimension and different chiral representation. In lattice discretizations which do not violate chiral symmetry this operator is multiplicatively renormalizable.
\item
Discretization effects of the $B_{\rm K}$ estimate at finite lattice spacing are $O(a)$; with staggered and Ginsparg-Wilson fermions they are $O(a^2)$. The traditional remedy of Symanzik improvement is not viable here, because of the large number of higher dimensional $O(a)$ counterterms required.
\end{enumerate}

The first of these problems has been dealt with in ref.~\cite{BK:WI}, by using  Ward identities, and in refs.~\cite{Dimopoulos:2006dm,Dimopoulos:2007cn}, by implementing twisted Wilson fermions~\cite{tmqcd:pap1}. In the latter case, the lattice fermion action consists of a twisted up-down fermion doublet (tmQCD) and a standard  (untwisted) Wilson strange fermion. A second possibility, valid only in the quenched approximation, is that of a tmQCD  discretization of a degenerate down-strange doublet.
The lack of mixing with other operators in both tmQCD variants is achieved through the mapping of the usual, parity-even $\Delta S = 2$ operator to its parity-odd counterpart, which is known to be multiplicatively renormalizable, even with Wilson fermions~\cite{Bernard:lat87,Doninetal:4fRIMOM}. Both formalisms have been applied in refs.~\cite{Dimopoulos:2006dm,Dimopoulos:2007cn}, combined with the Schr\"odinger functional renormalization and RG-running of ref.~\cite{ssf:vapav}.

In order to deal with the problem of improvement, one must ensure that all flavours are regularized in a tmQCD framework at maximal twist. In other words, the twist angle for all quark flavours must be tuned to $\pm \pi/2$, while the mapping from parity-even to parity-odd $\Delta S = 2$ operator must be preserved. As discussed in ref.~\cite{tmqcd:DIrule} this is not possible in the standard tmQCD formalism. A way round this problem was provided in ref.~\cite{FrezzoRoss2}, by using slightly different regularizations for sea and valence quarks. The former may be standard tmQCD, while the latter is the so-called Osterwalder-Seiler variant of tmQCD. Each valence quark is maximally twisted to $\pm \pi/2$. However, unlike standard tmQCD, the valence flavours are not combined into isospin doublets.
The four fermion operator consists of four distinct, maximally twisted valence flavours, three of which have twist angle with the same sign (say, $+\pi/2$) while the fourth twist angle has the opposite sign (say, $-\pi/2$). This combination of valence quarks ensures that the $\Delta S =2$ operator of interest is multiplicatively renormalizable and its $K^0 - \overline K^0$ matrix element is automatically improved; the same is true for $B_{\rm K}$.

It is not surprising that a price has to be paid for these advantages. In the setup described above, the $K^0$-meson consists of a strange/down valence quark - antiquark pair with, say, the same twist angle, while the $\overline K^0$-meson has a pair with opposite twist angles. This means that the two mesons have (pseudoscalar) masses which differ by $O(a^2)$ discretization effects. Although in principle this mass splitting vanishes in the continuum limit, it may be quite relevant at finite lattice spacing. Such effects have indeed been studied in the past (cf. refs~\cite{Jansen:2005cg,Abdel-Rehim:2006ve,Becirevic:2006ii}), as indirect manifestations of flavour symmetry breaking by tmQCD. In this work we have also performed a similar study of such breaking effects for the $K$-meson mass $m_{\rm K}$ and decay constant $f_{\rm K}$. A comparison of our results with those of ref.~\cite{Abdel-Rehim:2006ve} indicates that the presence of the Clover term in the action greatly reduces such flavour breaking systematics, in accordance with the findings of an earlier study.~\cite{Becirevic:2006ii} .


==> paper_parts/macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CUSTOM COMMANDS

\newcommand{\parbreak}{\vskip 0.15cm}

% Abbreviations for environment tags
%\newcommand{\ba}{\begin{array}}
%\newcommand{\ea}{\end{array}}

% References
\newcommand{\req}[1]{Eq.~(\ref{#1})}
\newcommand{\res}[1]{Section~\ref{#1}}
\newcommand{\reapp}[1]{Appendix~\ref{#1}}
\newcommand{\rep}[1]{\cite{#1}}
\newcommand{\refig}[1]{Fig.~\ref{#1}}
\newcommand{\ret}[1]{Table~\ref{#1}}

% Miscellaneous symbols
\newcommand{\dif}{{\rm d}}
%\newcommand{\Tr}{{\rm Tr}}
%\newcommand{\tr}{{\rm tr}}
\newcommand{\Pf}{{\rm Pf}}
\newcommand{\Id}{\mathbf{1}}
\newcommand{\pexp}{\mbox{P} \, \mbox{exp}}
\newcommand{\Per}[1]{\mathbf{S}_{#1}}
%\newcommand{\eps}{\varepsilon}
\newcommand{\ci}[1]{\boldsymbol{#1}}
\renewcommand{\Re}[1]{{\mathcal Re}\left\{#1\right\}}
\renewcommand{\Im}[1]{{\mathcal Im}\left\{#1\right\}}
\newcommand{\Dslash}{\relax{\kern+.25em / \kern-.70em D}}
\newcommand{\Dwd}{D_{\rm\tiny W}}
\newcommand{\arcsinh}{\rm arcsinh}
\newcommand{\arccosh}{\rm arccosh}
\newcommand{\arctanh}{\rm arctanh}

% Numerical sets / Groups
\newcommand{\Real}{\relax{\mathsf{\Gamma\kern-.35em R}}}
\newcommand{\Int}{\relax{\mathsf{Z\kern-.40em Z}}}
\newcommand{\Ztwo}{Z_2}
%\newcommand{\Zf}{Z_4}
\newcommand{\ZN}{Z_{\NC}}
\newcommand{\ZTN}{Z_{2\NC}}
\newcommand{\UO}{\mbox{U}(1)}
\newcommand{\SUT}{\mbox{SU}(2)}
\newcommand{\UT}{\mbox{U}(2)}
\newcommand{\SUt}{\mbox{SU}(3)}
\newcommand{\Ut}{\mbox{U}(3)}
\newcommand{\SUN}{\mbox{SU}(\NC)}
\newcommand{\UN}{\mbox{U}(\NC)}
\newcommand{\SUQ}{\mbox{SU}(Q)}
\newcommand{\UQ}{\mbox{U}(Q)}
%\newcommand{\SU}{\mbox{SU}}
%\newcommand{\CF}{C_{\rm F}}

% Scriptstyle fractions
\newcommand{\half}{{\scriptstyle{{1\over 2}}}}
\newcommand{\third}{{\scriptstyle{{1\over 3}}}}
\newcommand{\quart}{{\scriptstyle{{1\over 4}}}}
\newcommand{\sixth}{{\scriptstyle{{1\over 6}}}}
\newcommand{\eighth}{{\scriptstyle{{1\over 8}}}}
\newcommand{\sixteenth}{{\scriptstyle{{1\over 16}}}}
\newcommand{\twth}{{\scriptstyle{{1\over 12}}}}
\newcommand{\thalf}{{\scriptstyle{{3\over 2}}}}
\newcommand{\fhalf}{{\scriptstyle{{5\over 2}}}}
\newcommand{\tthird}{{\scriptstyle{{2\over 3}}}}
\newcommand{\fthird}{{\scriptstyle{{5\over 3}}}}
\newcommand{\ihalf}{{\scriptstyle{{i\over 2}}}}
\newcommand{\iquart}{{\scriptstyle{{i\over 4}}}}
\newcommand{\oneovN}{{\scriptstyle{{1\over \NC}}}}

% Colours, flavours, susies
%\newcommand{\NC}{N_c}
\newcommand{\NC}{N}
\newcommand{\NF}{N_f}
\newcommand{\NSS}{{\cal N}}

% Renormalisation schemes
%\newcommand{\MS}{{\rm MS}}
%\newcommand{\MSbar}{{\overline{\rm MS}}}
%\newcommand{\SF}{{\rm SF}}

% Renormalised, RGI and related quantities
%\newcommand{\gbar}{\kern1pt\overline{\kern-1pt g\kern-0pt}\kern1pt}
\newcommand{\gren}{g_{\rm R}}
\newcommand{\mbaref}[1]{m_{0, \rm #1}}
%\newcommand{\mbar}{\kern2pt\overline{\kern-1pt m\kern-1pt}\kern1pt}
\newcommand{\mbarf}[1]{\mbar_{\rm #1}}
\newcommand{\mren}[1]{m_{{\rm R} #1}}
\newcommand{\muren}[1]{\mu_{{\rm R} #1}}
\newcommand{\obar}[1]{\kern3pt\overline{\kern-2pt #1\kern-0pt}\kern1pt}
\newcommand{\oren}[1]{#1_{\rm R}}
\newcommand{\corrbar}[1]{\kern3pt\overline{\kern-2pt #1\kern-0pt}\kern1pt}
\newcommand{\corrren}[1]{#1_{\rm R}}
\newcommand{\lQCD}{\Lambda_{\rm\scriptscriptstyle QCD}}
\newcommand{\mrgi}{M}
\newcommand{\orgi}[1]{\hat #1}
%\newcommand{\orgi}[1]{#1_{\rm RGI}}
\newcommand{\msubt}{m_{\rm q}}
\newcommand{\mcrit}{m_{\rm cr}}
%\newcommand{\hopc}{\kappa_{\rm cr}}

\newcommand{\dstwo}{\scriptscriptstyle \Delta {\rm S} =2}

\newcommand{\oVA}[1]{#1_{\rm\scriptscriptstyle VA}}
\newcommand{\oAV}[1]{#1_{\rm\scriptscriptstyle AV}}
\newcommand{\oVV}[1]{#1_{\rm\scriptscriptstyle VV}}
\newcommand{\oAA}[1]{#1_{\rm\scriptscriptstyle AA}}

\newcommand{\oVApAV}[1]{#1_{\rm\scriptscriptstyle VA+AV}}
\newcommand{\oVAmAV}[1]{#1_{\rm\scriptscriptstyle VA-AV}}
\newcommand{\oSPpPS}[1]{#1_{\rm\scriptscriptstyle SP+PS}}
\newcommand{\oSPmPS}[1]{#1_{\rm\scriptscriptstyle SP-PS}}
\newcommand{\oVVpAA}[1]{#1_{\rm\scriptscriptstyle VV+AA}}
\newcommand{\oVVmAA}[1]{#1_{\rm\scriptscriptstyle VV-AA}}
\newcommand{\oSSpPP}[1]{#1_{\rm\scriptscriptstyle SS+PP}}
\newcommand{\oSSmPP}[1]{#1_{\rm\scriptscriptstyle SS-PP}}
\newcommand{\oTT}[1]{#1_{\rm\scriptscriptstyle TT}}
\newcommand{\oTtT}[1]{#1_{\rm\scriptscriptstyle T\tilde T}}
\newcommand{\oLL}[1]{#1_{\rm\scriptscriptstyle LL}}
\newcommand{\oRR}[1]{#1_{\rm\scriptscriptstyle RR}}
\newcommand{\oLR}[1]{#1_{\rm\scriptscriptstyle LR}}
\newcommand{\oRL}[1]{#1_{\rm\scriptscriptstyle RL}}

\newcommand{\oVApAVren}[1]{\kern3pt\overline{\kern-2pt #1\kern-0pt}\kern1pt_{\rm\scriptscriptstyle VA+AV;s}}

% Correlation functions
\newcommand{\fX}{f_{\rm\scriptscriptstyle X}}
\newcommand{\fP}{f_{\rm\scriptscriptstyle P}}
\newcommand{\fS}{f_{\rm\scriptscriptstyle S}}
\newcommand{\fA}{f_{\rm\scriptscriptstyle A}}
\newcommand{\fV}{f_{\rm\scriptscriptstyle V}}
\newcommand{\kX}{k_{\rm\scriptscriptstyle X}}
\newcommand{\kA}{k_{\rm\scriptscriptstyle A}}
\newcommand{\kV}{k_{\rm\scriptscriptstyle V}}
\newcommand{\kT}{k_{\rm\scriptscriptstyle T}}
\newcommand{\hT}{h_{\rm\scriptscriptstyle T}}

\newcommand{\FY}{F_{\rm\scriptscriptstyle Y}}
\newcommand{\FVA}{F_{\rm\scriptscriptstyle VA}}
\newcommand{\FAV}{F_{\rm\scriptscriptstyle AV}}
\newcommand{\FVV}{F_{\rm\scriptscriptstyle VV}}
\newcommand{\FAA}{F_{\rm\scriptscriptstyle AA}}

\newcommand{\hVApAV}{h_{\rm\scriptscriptstyle VA+AV}}
\newcommand{\hVAmAV}{h_{\rm\scriptscriptstyle VAmAV}}
\newcommand{\hSPpPS}{h_{\rm\scriptscriptstyle SP+PS}}
\newcommand{\hSPmPS}{h_{\rm\scriptscriptstyle SP-PS}}
\newcommand{\hTtT}{h_{\rm\scriptscriptstyle T\tilde T}}

% Z's, SSF's et rel.
\newcommand{\Zm}{Z_{\rm m}}
\newcommand{\ZP}{Z_{\rm\scriptscriptstyle P}}
\newcommand{\ZS}{Z_{\rm\scriptscriptstyle S}}
\newcommand{\ZA}{Z_{\rm\scriptscriptstyle A}}
\newcommand{\ZV}{Z_{\rm\scriptscriptstyle V}}
\newcommand{\ZT}{Z_{\rm\scriptscriptstyle T}}
\newcommand{\ZVApAV}[1]{Z_{\rm\scriptscriptstyle VA+AV #1}}
\newcommand{\ZVAmAV}[1]{Z_{\rm\scriptscriptstyle VA-AV #1}}
\newcommand{\ZSPpPS}[1]{Z_{\rm\scriptscriptstyle SP+PS #1}}
\newcommand{\ZSPmPS}[1]{Z_{\rm\scriptscriptstyle SP-PS #1}}
\newcommand{\ZTtT}[1]{Z_{\rm\scriptscriptstyle T\tilde T #1}}
\newcommand{\ZtotVApAV}[1]{\mathcal{Z}_{\rm\scriptscriptstyle VA+AV #1}}
\newcommand{\ZtotVAmAV}[1]{\mathcal{Z}_{\rm\scriptscriptstyle VA-AV #1}}
\newcommand{\ZtotSPpPS}[1]{\mathcal{Z}_{\rm\scriptscriptstyle SP+PS #1}}
\newcommand{\ZtotSPmPS}[1]{\mathcal{Z}_{\rm\scriptscriptstyle SP-PS #1}}
\newcommand{\ZtotTtT}[1]{\mathcal{Z}_{\rm\scriptscriptstyle T\tilde T #1}}

\newcommand{\zbar}{\kern3pt\overline{\kern-2pt Z\kern-0pt}\kern1pt}
\newcommand{\zrgi}{\hat Z}
\newcommand{\zbarVApAV}[1]{\kern3pt\overline{\kern-2pt Z\kern-0pt}\kern1pt_{\rm\scriptscriptstyle VA+AV #1}}
\newcommand{\zrgiVApAV}[1]{\hat Z_{\rm VA+AV #1}}

\newcommand{\sigmaP}{\sigma_{\rm\scriptscriptstyle P}}
\newcommand{\sigmaT}{\sigma_{\rm\scriptscriptstyle T}}
\newcommand{\SigmaP}{\Sigma_{\rm\scriptscriptstyle P}}
\newcommand{\SigmaT}{\Sigma_{\rm\scriptscriptstyle T}}

\newcommand{\sigVApAV}[1]{\sigma_{\rm\scriptscriptstyle VA+AV #1}}
\newcommand{\sigVAmAV}[1]{\sigma_{\rm\scriptscriptstyle VA-AV #1}}
\newcommand{\sigSPpPS}[1]{\sigma_{\rm\scriptscriptstyle SP+PS #1}}
\newcommand{\sigSPmPS}[1]{\sigma_{\rm\scriptscriptstyle SP-PS #1}}
\newcommand{\sigTtT}[1]{\sigma_{\rm\scriptscriptstyle T\tilde T #1}}

\newcommand{\SigVApAV}[1]{\Sigma_{\rm\scriptscriptstyle VA+AV #1}}
\newcommand{\SigVAmAV}[1]{\Sigma_{\rm\scriptscriptstyle VA-AV #1}}
\newcommand{\SigSPpPS}[1]{\Sigma_{\rm\scriptscriptstyle SP+PS #1}}
\newcommand{\SigSPmPS}[1]{\Sigma_{\rm\scriptscriptstyle SP-PS #1}}
\newcommand{\SigTtT}[1]{\Sigma_{\rm\scriptscriptstyle T\tilde T #1}}

\newcommand{\PISigVApAV}[1]{\tilde\Sigma_{\rm\scriptscriptstyle VA+AV #1}}

\newcommand{\UVApAV}[1]{U_{\rm\scriptscriptstyle VA+AV #1}}

\newcommand{\gamVApAV}[1]{\gamma_{\rm\scriptscriptstyle VA+AV #1}}
\newcommand{\gamVAmAV}[1]{\gamma_{\rm\scriptscriptstyle VA-AV #1}}
\newcommand{\gamSPpPS}[1]{\gamma_{\rm\scriptscriptstyle SP+PS #1}}
\newcommand{\gamSPmPS}[1]{\gamma_{\rm\scriptscriptstyle SP-PS #1}}
\newcommand{\gamTtT}[1]{\gamma_{\rm\scriptscriptstyle T\tilde T #1}}

\newcommand{\lmax}{L_{\rm max}}
\newcommand{\lmin}{L_{\rm min}}
\newcommand{\mumax}{\mu_{\rm max}}
\newcommand{\mumin}{\mu_{\rm min}}

% O(a) improvement
%\newcommand{\Oa}{\mbox{O}(a)}
%\newcommand{\Oasq}{\mbox{O}(a^2)}
\newcommand{\Ogsqa}{\mbox{O}(g_0^2 a)}
\newcommand{\Ogqa}{\mbox{O}(g_0^4 a)}
\newcommand{\icsw}{c_{\rm sw}}
\newcommand{\ict}{c_{\rm t}}
\newcommand{\icttil}{\tilde c_{\rm t}}
\newcommand{\icP}{c_{\rm\scriptscriptstyle P}}
\newcommand{\icA}{c_{\rm\scriptscriptstyle A}}
\newcommand{\icT}{c_{\rm\scriptscriptstyle T}}
\newcommand{\icV}{c_{\rm\scriptscriptstyle V}}
\newcommand{\ibP}{b_{\rm\scriptscriptstyle P}}
\newcommand{\ibA}{b_{\rm\scriptscriptstyle A}}
\newcommand{\ibT}{b_{\rm\scriptscriptstyle T}}
\newcommand{\ibV}{b_{\rm\scriptscriptstyle V}}
\newcommand{\ibm}{b_{\rm m}}

% Boldface and calligraphic capitals
\newcommand{\bA}{{\mathbf{A}}}
\newcommand{\bB}{{\mathbf{B}}}
\newcommand{\bC}{{\mathbf{C}}}
\newcommand{\bD}{{\mathbf{D}}}
\newcommand{\bE}{{\mathbf{E}}}
\newcommand{\bF}{{\mathbf{F}}}
\newcommand{\bG}{{\mathbf{G}}}
\newcommand{\bH}{{\mathbf{H}}}
\newcommand{\bI}{{\mathbf{I}}}
\newcommand{\bJ}{{\mathbf{J}}}
\newcommand{\bK}{{\mathbf{K}}}
\newcommand{\bL}{{\mathbf{L}}}
\newcommand{\bM}{{\mathbf{M}}}
\newcommand{\bN}{{\mathbf{N}}}
\newcommand{\bO}{{\mathbf{O}}}
\newcommand{\bP}{{\mathbf{P}}}
\newcommand{\bQ}{{\mathbf{Q}}}
\newcommand{\bR}{{\mathbf{R}}}
\newcommand{\bS}{{\mathbf{S}}}
\newcommand{\bT}{{\mathbf{T}}}
\newcommand{\bU}{{\mathbf{U}}}
\newcommand{\bV}{{\mathbf{V}}}
\newcommand{\bW}{{\mathbf{W}}}
\newcommand{\bX}{{\mathbf{X}}}
\newcommand{\bY}{{\mathbf{Y}}}
\newcommand{\bZ}{{\mathbf{Z}}}
\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cQ}{{\cal Q}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}
\newcommand{\cZ}{{\cal Z}}

% Boldface three-vectors and funny caps for momenta
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vt}{\mathbf{t}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\vk}{\mathbf{k}}
\newcommand{\vl}{\mathbf{l}}
\newcommand{\vn}{\mathbf{n}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vzero}{\mathbf{0}}
%\newcommand{\ring}[1]{\mathaccent"7017 #1}

\newcommand{\scrA}{{\rm\scriptscriptstyle A}}
\newcommand{\scrP}{{\rm\scriptscriptstyle P}}
\newcommand{\scrV}{{\rm\scriptscriptstyle V}}


==> paper_parts/results.tex <==
\section{Results}
\label{sec:results}

We have obtained quenched results at three values of the gauge coupling, namely $\beta=6.0, ~6.1, ~6.2$. At each coupling we have tuned the quark masses $a\mu$ to a couple of values which are close to half the strange quark mass, so as to simulate charged K-mesons with degenerate flavours.
The values of $\kappa_{\rm cr}$, used in the simulations in order to achieve maximal twist, are collected in Table 3 of ref.~\cite{Dimopoulos:2007cn}. The renormalization constants, improving coefficients and the ratio $r_0/a$ used in this work have been gathered in Appendix A of ref.~\cite{Dimopoulos:2006dm}. We use several of these when computing physical quantities, usually expressed in units of $r_0$ in the present work.

The details of the runs are reported in Table~\ref{tab:runs}. The lattice size is $L^3 \times T$ with standard Schr\"odinger Functional boundaries. The lattice calibration, expressed in terms of $a/2r_0$, is that of ref.~\cite{Dimopoulos:2006dm}. In the Table we also show the plateau (in units of $x_0/2r_0$) for which the ground state of our correlation functions (i.e. the K-meson) has been isolated. As this exploratory study aims at qualitative numerical indications, rather than precision measurements, our statistics are rather low.
\begin{table}[!h]
\small
\begin{center}
\begin{tabular}{ccccccc}
\hline \hline
$\beta$   & $\frac{a}{2r_0}$  & (L,~ T)   &  $[\frac{x_0^{min}}{2r_0},\frac{x_0^{max}}{2r_0}$] & $N_{\mbox {meas}}$   &  $a\mu$ & dataset  \\ 
\hline
&&&&&&  \\
6.0       & 0.0931   & (24,~ 48) &   [1.30,3.17]       &  100        &  0.0135  & I  \\ 
6.0       & 0.0931   & (24,~ 48) &   [1.30,3.17]       &  100        &  0.0115  & II \\
&&&&&& \\ 
6.1       & 0.0789   & (24,~ 60) &   [1.26,3.47]       &  100        &  0.0125  & I \\ 
6.1       & 0.0789   & (24,~ 60) &   [1.26,3.47]       &  100        &  0.0110  & II\\
&&&&&&  \\
6.2       & 0.0677   & (32,~ 72) &   [1.35,3.52]       &  50         &  0.0105  & I \\ 
6.2       & 0.0677   & (32,~ 72) &   [1.35,3.52]       &  50         &  0.0090  & II \\
&&&&&&  \\
\hline \hline
\end{tabular} \vspace*{0.3cm}
\caption{Details of the runs for three values of the gauge coupling.}
\label{tab:runs}
\end{center}
\end{table}

\subsection{Discretization effects between tm and OS quantities}

All observables computed in this work are obtained from the large
time asymptotic limit of operator correlation functions with
Schr\"odinger functional (SF) boundary conditions.
The notation is standard, following closely that adopted e.g.
in  ref.~\rep{Dimopoulos:2006dm}. For instance, $f_\scrA$ ($f^\prime_\scrA$) denotes
the Schr\"odinger functional correlation with a fermionic operator
$A_0$ in the bulk and a time-boundary pseudoscalar
operator $\bar \zeta_s \gamma_5 \zeta_d$ at time-slice $x_0=0$ ($x_0=T$).
All such correlation functions are properly (anti)symmetrized in time,
when used to extract quark masses, effective pseudoscalar masses
and decay constants. 

We have measured pseudoscalar effective masses $a M (x_0)$, both in the
tm and OS framework:
\begin{eqnarray}
a M^{\rm tm} (x_0) = \dfrac{1}{2} 
\ln \Bigg [ \dfrac{ f_{\scrV}^{\rm tm} (x_0-a)}{f_\scrV^{\rm tm} (x_0+a)} \Bigg ] \,\, ;
\qquad
a M^{\rm OS} (x_0) = \dfrac{1}{2} 
\ln \Bigg [ \dfrac{ f_{\scrA}^{\rm OS} (x_0-a)}{f_\scrA^{\rm OS} (x_0+a)} \Bigg ] 
\,\, .
\label{eq:effmass}
\end{eqnarray}
In Table~\ref{tab:mK} we show the results of the pseudoscalar meson masses from both regularisations.
Recall that the physical value of the Kaon mass in units of $r_0$ is $r_0 M_{\rm K} = 1.2544$. Therefore, 
for all three $\beta$-values, the K-meson decay constant $F_{\rm K}$ and the bag parameter $B_{\rm K}$  discussed below, are obtained through short ``interpolations" between two points.
We also show in Table~\ref{tab:mK} that the relative mass splitting, defined by
\begin{equation} \label{Ratio}
R_M =  \dfrac{(r_0 M^{\rm OS})^2 - (r_0 M^{\rm tm})^2}{(r_0 M^{\rm tm})^2} \,\,\, ,
\end{equation}
decreases with decreasing lattice spacing. This is a clear evidence that  the mass splitting is a discretisation effect. 

The next step consists in comparing our results to those of other collaborations, by examining the pseudoscalar meson mass splitting in units of $r_0$:
\begin{equation}
\Delta (r_0^2 M^2) \,\, \equiv \,\, [ r_0 M^{\rm OS} ]^2 - [ r_0 M^{\rm tm} ]^2 \,\,\, .
\end{equation}
In Fig.~\ref{fig:mass-split1} we plot our data against those of ref.~\cite{Abdel-Rehim:2006ve}, which are also $O(a)$-improved, having been obtained with the maximally twisted Wilson action, {\it without a Clover term}, and an ``optimal" $\kappa_{\rm cr}$. The mass splitting of our results is significantly smaller\footnote{In ref.~\cite{Abdel-Rehim:2006ve} the pseudoscalar masses $a M^{\rm tm}$ and  $a M^{\rm OS}$ are tabulated. Since these quantities are correlated, it is impossible to compute the error of $\Delta (r_0^2 M^2)$ from those of the two masses. We therefore quote for $\Delta (r_0^2 M^2)$ the same (relative) error as the bigger (relative) error of the two masses.}.  We attribute this to the inclusion of the Clover term in the action. This effect, already seen in ref.~\cite{Becirevic:2006ii} at $\beta = 6.0$, is confirmed here for more lattice spacings. As the data of ref.~\cite{Abdel-Rehim:2006ve} clearly indicate, this splitting depends weakly upon the quark mass values. We expect a similarly weak mass dependence in our case.
It is interesting to note that the authors of~\cite{Abdel-Rehim:2006ve} also find that their results are in good agreement with those of ref.~ref.~\cite{Jansen:2005cg}, obtained with a maximally twisted Wilson action (without a Clover term) and a slightly different method for computing the ``optimal" $\kappa_{\rm cr}$. We also point out that this mass splitting has been recently studied in an unquenched $N_f=2$ framework, with a maximally tmQCD action without a Clover term; see ref.~\cite{Dimopoulos:2008hb}. In this preliminary work, pronounced $R_M$ values of up to about $50\%$ have been reported.
\vskip 0.0cm
\begin{figure}[!ht]
{\includegraphics[scale=0.50, angle=-90]{comparison_I.ps}}
%\epsfig{figure=comparison_I.ps, angle=-90, width=13.6 true cm}
\vskip -0.5cm
\begin{center}
\caption{Square-mass splitting between tm and OS pseudoscalar mesons, as a function of the summed renormalized twisted mass parameters of their valence quarks.}
\label{fig:mass-split1}
\end{center}
\end{figure}
\vskip 0.0cm
\begin{figure}[!ht]
{\includegraphics[scale=0.50, angle=-90]{comparison_II.ps}}
%\epsfig{figure=comparison_II.ps, angle=-90, width=13.6 true cm}
\vskip -0.5cm
\begin{center}
\caption{Square-mass splitting between tm and OS pseudoscalar mesons, as a function of the lattice spacing squared.}
\label{fig:mass-split2}
\end{center}
\end{figure}
\vskip 0.0cm
\begin{figure}[!ht]
{\includegraphics[scale=0.50, angle=-90]{comparison_III.ps}}
%\epsfig{figure=comparison_III.ps, angle=-90, width=13.6 true cm}
\vskip -0.5cm
\begin{center}
\caption{Square-mass splitting between tm and OS pseudoscalar mesons, as a function of the lattice spacing to the fourth power.}
\label{fig:mass-split3}
\end{center}
\end{figure}

In Fig.~\ref{fig:mass-split2} we plot $\Delta (r_0^2 M^2)$ against the lattice spacing squared, for the present work and ref.~\cite{Abdel-Rehim:2006ve}. In both cases this cutoff effect is decreasing with the lattice spacing, with the intercept of our results clearly smaller (if negative). However, it does not vanish in the continuum limit, as expected. Most peculiarly, the vanishing of $\Delta (r_0^2 M^2)$ in the continuum appears to be supported by our data if plotted against $a^4$; cf. Fig.~\ref{fig:mass-split3}. We have currently no plausible explanation for this $a^4$ behaviour of our data. Note that the results of  ref.~\cite{Abdel-Rehim:2006ve}, plotted against $a^4$, still display a non-zero intercept.

\begin{table}[!h]
\small
\begin{center}
\begin{tabular}{ccccc}
\hline \hline
$\beta$     &   dataset   &   $r_0M^{\rm tm}$   &  $r_0M^{\rm OS}$   &  $R_M$ in $\%$ \\
\hline
 6.0        &    I        &    1.255(5)      &   1.346(8)       &   15        \\
 6.0        &    II       &    1.169(5)      &   1.267(9)       &   17        \\  
 &&&& \\
 6.1        &    I        &    1.295(6)      &   1.349(8)       &   8       \\
 6.1        &    II       &    1.222(6)      &   1.279(8)       &   9       \\
 &&&& \\
 6.2        &    I        &    1.268(8)      &   1.301(10)      &   5       \\
 6.2        &    II       &    1.182(8)      &   1.217(10)      &   6       \\
&&&&  \\
\hline \hline
\end{tabular} \vspace*{0.3cm}
\caption{Pseudoscalar masses of tm and OS type and their mass splitting as defined in Eq~(\ref{Ratio}).  }
\label{tab:mK}
\end{center}
\end{table}

A similar analysis is performed for the pseudoscalar meson decay constants. In the Schr\"odinger functional framework they are obtained from the axial current correlation functions $f_{\scrA_{\rm R}}$, properly normalized by the boundary-to-boundary correlation function $f_1$; see~\rep{mbar:pap2} for details. For the maximally twisted tm and OS cases under investigation, the specific expressions
are (in the large time asymptotic regime):
\begin{eqnarray}
F^{\rm tm}  &\approx& 2 (M^{\rm tm} L^3)^{-1/2} 
\exp[(x_0 - T/2)M^{\rm tm}] \dfrac{- i Z_V f_{\scrV}^{\rm tm}(x_0)}{\sqrt{f_1^{\rm tm}}}\,\, ,
\label{eq:dc-ud}
\\
F^{\rm OS} &\approx& 2 (M^{\rm OS} L^3)^{-1/2} \exp[(x_0 - T/2)M^{\rm OS}]
\dfrac{Z_A f_\scrA^{\rm OS}(x_0)}{\sqrt{f_1^{\rm OS}}}\ .
\label{eq:dc-sc}
\end{eqnarray}
The quantities $F^{\rm tm}$ and $F^{\rm OS}$ are obtained from these
expressions in the range of $x_0 \gg 0$ in which the
pseudoscalar effective masses have been extracted.
% refs.~\cite{impr:pap4}.
\parbreak
A further method for computing $F$ is based on the PCVC relation, expressed in terms of Schr\"odinger
functional correlation functions:
\begin{equation}
-M Z_V f_\scrV^{\rm tm} (x_0) = 2 i \mu f_{\scrP}^{\rm tm} (x_0)\ .
\label{eq:exctPCVC2}
\end{equation}
The corresponding decay constant is computed as
\begin{eqnarray}
F^{\rm PCVC}  &\approx& - 4 \dfrac{\mu}{M^{\rm tm}}
(M^{\rm tm} L^3)^{-1/2} \exp[(x_0 - T/2) M^{\rm tm}] 
\dfrac{f_{\scrP}^{\rm tm}(x_0)}{\sqrt{f_1^{\rm tm}}}\ .
\label{eq:dc-ud2}
\end{eqnarray}

In Table~\ref{tab:fK} we show out results for the pseudoscalar decay constants. These 
values are in a general agreement with the corresponding estimates in Tables 6 and 7 of 
ref.~\cite{Dimopoulos:2007cn}, but the errors are bigger, due to reduced statistics\footnote{The quantities $r_0 F^{\rm PCVC}$ and $r_0 F^{\rm tm}$ have also been computed in
ref.~\cite{Dimopoulos:2007cn}. However these computations had been performed at significantly 
heavier quark masses and extrapolated to the Kaon mass value. This accounts for the $4\%$
difference between these results and ours at $\beta = 6.0$; this difference decreases with increasing $\beta$.}. 
The principal observation is that $F^{\rm tm}$ and  $F^{\rm OS}$ are compatible within errors;
thus discretization effects turn out to be small. 

\begin{table}[!h]
\small
\begin{center}
\begin{tabular}{ccccc}
\hline \hline
$\beta$     &   dataset   &   $r_0F^{\rm PCVC}$   &  $r_0F^{\rm tm}$   & 
$r_0F^{\rm OS}$ \\
\hline
 6.0        &    I        &   0.407(7)     &  0.411(6)      &  0.412(12)       \\
 6.0        &    II       &   0.397(6)     &  0.401(6)      &  0.408(13)       \\  
            &  $r_0M_{\rm K}$    &   0.407(6)    &   0.411(6)     &   0.412(12)       \\
 &&&& \\
 6.1        &    I        &   0.415(8)    &  0.419(8)       &  0.410(9)       \\
 6.1        &    II       &   0.407(8)    &  0.411(8)       &  0.404(10)       \\
            &  $r_0M_{\rm K}$   &   0.411(8)    &   0.415(8)      &  0.407(10)       \\
 &&&& \\ 
 6.2        &    I        &   0.417(12)    &  0.420(11)     &  0.419(14)       \\
 6.2        &    II       &   0.408(11)    &  0.411(11)     &  0.412(14)       \\
            &  $r_0M_{\rm K}$   &   0.416(11)    &   0.419(11)    &   0.418(14)       \\
 &&&& \\
\hline \hline
\end{tabular} \vspace*{0.3cm}
\caption{Pseudoscalar decay constants obtained from PCVC, and the axial current of tm
and OS type. We also show the interpolations at the physical K-meson point.}
\label{tab:fK}
\end{center}
\end{table}

\subsection{Improved $B_{\rm K}$ parameter}

The main result of this work is the computation of an automatically improved $B_{\rm K}$ parameter, on the lines of ref.~\cite{FrezzoRoss2}. The four fermion operator of interest is
\begin{equation}
Q_{VV+AA}^{\rm cont} = [ \bar s \gamma_\mu d ] [ \bar s \gamma_\mu d ]
+[ \bar s \gamma_\mu \gamma_5 d ] [ \bar s \gamma_\mu \gamma_5 d ]  \,\, .
\end{equation}
On the lattice, we opt to discretize this operator as proposed in ref.~\cite{FrezzoRoss2};
i.e. it is expressed in terms of current products made of both tm and OS type, at maximal twist:
\begin{equation}
Q_{VA+AV}^{\rm tm-OS} = 
[ \bar s \gamma_\mu d ]^{\rm tm} [ \bar s \gamma_\mu \gamma_5 d ]^{\rm OS}
+ [ \bar s \gamma_\mu \gamma_5 d ]^{\rm tm} [ \bar s \gamma_\mu d ]^{\rm OS}  \,\, .
\label{eq:VA+AV}
\end{equation}
The relation between the lattice and continuum operators, up to discretization effects, is
\begin{equation}
Q_{VV+AA}^{\rm cont} = [Q_{VA+AV}^{\rm tm-OS}]_{\rm R} = Z_{VA+AV} Q_{VA+AV}^{\rm tm-OS}
\end{equation}
The main reason behind using this mixed tm-OS formalism is the fact that in this way the $B_{\rm K}$ matrix element, computed with (twisted) Wilson fermions, is both automatically improved and multiplicatively renormalizable.

$B_{\rm K}$ is obtained form the ratio
\begin{equation}
R_{B_{K}} = \dfrac{iZ_{VA+AV} F^{VA+AV}}{(8/3) [iZ_V f_V^{\rm tm}] ~ [Z_A f_A^{'\rm OS}]} \,\, ,
\end{equation}
where $F^{VA+AV}$ is the Schr\"odinger Functional correlation function with 
the four fermion operator of eq.~(\ref{eq:VA+AV}) in the bulk and the usual boundary sources
at the time edges. Note that these sources are of tm type at time-slice $x_0 = 0$ and of OS type at 
time-slice $x_0 = T$. Thus, away from the time boundaries, the correlation function $F^{VA+AV}$ displays an asymptotic behaviour of the form $\exp[-m^{\rm tm} x_0] \exp[-m^{\rm OS} (T-x_0)]$. 
In order to match this choice and cancel the exponentials, the denominator consists of a correlation function $f_V^{\rm tm}$ of the tm type, involving the $x_0 = 0$ boundary, and a correlation function
$f_A^{'\rm OS}$ of the OS-type, involving the $x_0 = T$ boundary. The axial and vector currents in these correlation functions are the corresponding tm and OS twisted versions of the axial current; 
cf. eqs.~(\ref{eq:Atm}),~(\ref{eq:AOS}). In our analysis we have also considered the symmetric situation with tm and OS sources exchanged and the denominator of the above equation adjusted accordingly.
The $B_{\rm K}$ result quoted below is the average of the two estimates thus obtained. 
The quality of our raw results for $R_{B_{K}}$ are shown in  Fig.~\ref{fig:BKplateau}.

\begin{figure}[!h]
\begin{center}
{\includegraphics[scale=0.50, angle=-90]{BK_plateaux.ps}}
\caption[]{The ratio $R_{B_{K}}(\rm RGI)$ as a function of time, for three values of the gauge coupling.
The data for $\beta=6.0$ and 6.1 have been shifted for clarity.  The straight lines indicate the $B_{\rm K}$ averages and the extension of the plateau.
}
\label{fig:BKplateau}
\end{center}
\end{figure}


At large time separations from the boundary, the bare $B_{\rm K}$ estimate is automatically improved. 
The renormalization constant $Z_{VA+AV}$ is known non-perturbatively from ref.~\cite{ssf:vapav}. As it is computed in the chiral limit but is not improved, it suffers from $O(a \Lambda_{\rm QCD})$ discretization effects. These are not expected to dominate the scaling behaviour of $B_{\rm K}$.


\begin{table}[!h]
\small
\begin{center}
\begin{tabular}{ccccc}
\hline \hline
$\beta$     &   dataset   &   $B_{\rm K}^{\rm RGI, tm-OS}$   &   $B_{\rm K}^{RGI, \pi/2}$   &
$B_{\rm K}^{RGI, \pi/4}$ \\
\hline
 6.0        &    I        &   0.772(10)(9)     &  &             \\
 6.0        &    II       &   0.753(12)(9)     &  &               \\
            &  $r_0M_{\rm K}$   &   0.772(10)(9)[14] &  0.911(22)     &   0.926(13)       \\
 &&&&\\
 6.1        &    I        &   0.762(12)(9)      &  &               \\
 6.1        &    II       &   0.746(13)(9)      &  &              \\
             &  $r_0M_{\rm K}$    &   0.753(12)(9)[15] &   0.824(26)       &  0.843(13)         \\
 &&&& \\
 6.2        &    I        &   0.758(12)(9)    &   &         \\
 6.2        &    II       &   0.742(13)(9)    &   &           \\
             &  $r_0M_{\rm K}$    &   0.756(12)(9)[15]    &0.828(30)       & 0.798(14)         \\
 &&&& \\
\hline \hline
\end{tabular} \vspace*{0.3cm}
\caption{Comparison of the $B_{\rm K}^{\rm RGI}$ results of the present work to those of
ref.~\cite{Dimopoulos:2007cn}. The errors quoted for $B_{\rm K}^{\rm RGI, tm-OS}$ are, in order
of appearance: (i) statistical, (ii) uncertainty due to the renormalization constants $Z_{VA+AV}$,
$Z_A$ and $Z_V$, (iii) total error.
 }
\label{tab:BK}
\end{center}
\end{table}


In Table~\ref{tab:BK} we list our $B_{\rm K}^{\rm RGI}$ estimates and compare them to those of ref.~\cite{Dimopoulos:2007cn}. We remind the reader that the latter had been computed in two distinct frameworks: (i) the so-called $\pi/2$ case, consisting of a maximally twisted down quark and a non-twisted strange one and (ii)  the so-called $\pi/4$ case, in which down and strange flavours were in the same isospin doublet with a twist angle $\pi/4$. In both frameworks we have quarks which are not maximally twisted and this implies that the results of ref.~\cite{Dimopoulos:2007cn} are not improved.  
Although it is clear from this comparison that the present improved $B_{\rm K}$ estimate has a much better
scaling behaviour, we wish to draw the reader's attention to a subtlety. This consists in the fact that
the unimproved $B_{\rm K}$ estimates of ref.~\cite{Dimopoulos:2007cn} were obtained with Symanzik-improved axial currents in the denominator, which contained the term $a c_A \partial_0 P$. Thus, the comparison between our present results (which only suffer from mild $O(a \Lambda_{\rm QCD})$ discretization errors and $O(a^2 \mu^2)$ ones) and the older unimproved ones is somewhat intricate.

%In order to avoid
%any arbitrariness of this kind, when comparing the older unimproved results to the present ones,
%we also compute the ratio of the four fermion matrix elements:
%\begin{eqnarray}
%R & = & \frac{ F^{VA+AV,\pi/2}}{ F^{VA+AV,\rm tm-OS}}
%\end{eqnarray}
%This ratio is free of the $B_{\rm K}$ denominators and the uncertainties that may arise in the axial
%current definition. Moreover, the renormalization constant $Z_{VA+AV}$ cancels in the ratio.
%The numerator of $R$ is characterized by $O(a)$ discretization effects, whereas for
%the denominator these effects are $O(a^2)$. Thus $R$ should highlight the improved approach to
%the continuum limit of our $B_{\rm K}$ estimate. DATA AND FIGURE HERE!

\begin{figure}[!h]
\begin{center}
{\includegraphics[scale=0.50,angle=-0]{BK_comparison_NPB.ps}}
\caption[]{The scaling behaviour of the new $B_{\rm K}$ estimate and the comparison with the old ones.
We have retained the same scale as in Fig.~7 of ref.~\cite{Dimopoulos:2007cn}.}
\label{scaling}
\end{center}
\end{figure}


In Fig.~\ref{scaling} we show the scaling bahaviour of our new estimates of  $B_{\rm K}^{\rm RGI, tm-OS}$ in comparison with the values given in ref.~\cite{Dimopoulos:2007cn}. 
%Note that  the scaling behaviour is presented as a function of $a/2r_0$ because the results of ref.~\cite{Dimopoulos:2007cn} are non-improved. 


A linear fit of our $B_{\rm K}^{RGI, ~\mbox{imp}}$ data  with respect to $a^2$ would give the following continuum result:
$$B_{\rm K}^{RGI, ~\mbox{imp}} = 0.733(35) ~~~ (\chi^2/dof = 0.26) $$ 
which compares nicely with our pubblished value: $B_{\rm K}^{RGI} = 0.735(71)$ of ref.~\cite{Dimopoulos:2007cn}.





==> paper_parts/title.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TITLE

\begin{titlepage}

%%% Preprint numbers %%%

\vspace*{-30truemm}
\begin{flushright}
%ROM2F/2007-03\\
%MS-TP-07-1\\
%CERN-PH-TH/2007-018\\
%MKPH-T-07-03\\ 
%TRINLAT-07/03\\
\vspace{5truemm}
{\large December 2008}
\end{flushright}
\vspace{5truemm}

%%% Title and authors %%%

\centerline{\Bigrm $B_{\rm K}$-parameter from Osterwalder-Seiler tmQCD quarks}
\centerline{\Bigrm and mass-splitting discretization effects}
\centerline{\Bigrm  }
\vskip 9 true mm
\begin{center}
\epsfig{figure=./alpha_color_60.ps, width=22 true mm}\\
\end{center}
\vskip -2 true mm
\centerline{\bigrm  P.~Dimopoulos$^a$, H.~Simma$^{b,c}$ and A.~Vladikas$^d$}
\vskip 4 true mm
\centerline{\it $^a$ Dipartimento di Fisica, Universit\`a di Roma ``Tor
  Vergata''}
\centerline{\it Via della Ricerca Scientifica 1, I-00133 Rome, Italy}
\vskip 3 true mm
\centerline{\it $^b$ DESY, Platanenallee 6, D-15738 Zeuthen, Germany}
\vskip 3 true mm
\centerline{\it $^c$ Dipartimento di Fisica, Universit\'a di Milano Bicocca,}
\centerline{\it Piazza della Scienza 3, I-20126 Milano, Italy}
\vskip 3 true mm
\centerline{\it $^d$ INFN, Sezione di ``Tor Vergata"}
\centerline{\it c/o Dipartimento di Fisica, Universit\`a di Roma ``Tor
  Vergata''}
\centerline{\it Via della Ricerca Scientifica 1, I-00133 Rome, Italy}

\vskip 10 true mm

%%% Abstract %%%

\thicktablerule
\vskip 3 true mm
\noindent{\tenbf Abstract}
\vskip 1 true mm
\noindent
{\tenrm  We apply an Osterwalder-Seiler version of twisted mass QCD to a study of the $B_{\rm K}$ parameter, in which three of the four quark fields of the relevant $\Delta S =2$ operator are maximally twisted with the same twist angle, while the fourth one has a twist angle of opposite sign. It is known that this ensures automatic improvement of the bare $K^0$-$\overline K^0$ operator matrix element and multiplicative renormalization of the  $\Delta S =2$ operator, at the price of breaking the $K^0$-$\overline K^0$ degeneracy by discretization effects. In this way, two dominant systematic errors of the $B_{\rm K}$ determination with Wilson fermions are kept under control. We perform a feasibility study and find, in the quenched approximation, a significant improvement of the scaling behaviour of $B_{\rm K}$, compared to earlier standard tmQCD determinations. Moreover, we study in detail the $K^0$-$\overline K^0$ mass splitting that characterizes this approach and confirm that it is greatly reduced in a maximally twisted theory with a Clover term in the fermion action.}
\vskip 3 true mm
\thicktablerule
%\vspace{10truemm}
\eject
\end{titlepage}



==> paper_parts/tm-OS.tex <==
\section{Twisted and Osterwalder-Seiler valence quarks}
\label{sec:tmQCD-gen}

The setup of our formalism follows very closely that of  ref.~\cite{FrezzoRoss2}. Each valence
quark field $\psi_f$ (the subscript labels flavour) is discretized by a fermionic action
of the form
\begin{align}
 \label{tmQCD_action2}
 S_f = a^4 \sum_x \,\,  \ {\bar \psi_f}(x) \big [ D_{\rm w} + m_f + i\gamma_5 \mu_{0,f} \big ]
 \psi_f(x) \,\,  ,
\end{align}
where $D_{\rm w}$ is the standard Dirac-Wilson fermion matrix (with a Clover term). The Wilson plaquette action is the regularization of the pure gauge sector of the theory. In this work
all flavours are degenerate; this is only a matter of choice. As our simulations are performed in the quenched approximation, we will ignore issues concerning the lattice regularization of the sea quarks; see \cite{FrezzoRoss2} for a related discussion.

Let us consider quark bilinear operators with distinct flavours. We distinguish two cases, depending on the relative sign of the twisted mass terms (or equivalently, the twist angle) of these flavours. With $\Gamma$ denoting any Dirac matrix and $\bar f(x)$, $g(x)$ quark fields of the corresponding flavour,
a quark bilinear operator of the form
\begin{align}
Q_{\Gamma,fg}^{\rm tm}(x) \,\,\, = \,\,\, \bar f(x) \,\, \Gamma \,\, g(x)
 \end{align}
is said to be of ``twisted mass" (tm) type, if the corresponding twisted mass terms have opposite signs
(i.e. $\mu_f = - \mu_g$). In this case the two flavours may be grouped in a doublet, with a mass term of
the form $i\mu\gamma_5 \tau^3$, corresponding to the standard tmQCD formalism ($\tau^3$ is the Pauli isospin matrix). A second possibility is that  of $\mu_f = \mu_g$; this will be referred to as the
Osterwalder-Seiler (OS) case. Operators are then denoted by
\begin{align}
Q_{\Gamma,fg}^{\rm OS}(x) \,\,\, = \,\,\, \bar f(x) \,\, \Gamma \,\, g(x) \,\, .
 \end{align}
The OS discretization is only applicable to valence quarks. Sea quarks,
if regularized by the tmQCD lattice action, must be organized in doublets, with a flavour non-singlet
twisted mass term $i\mu\gamma_5 \tau^3$, in order to avoid the generation of unwanted anomalies.
Thus, the implementation of OS valence flavours is a mixed action formulation, with inevitable
unitarity violation, at finite lattice spacing.

The specific continuum operators of interest are $P_{ds}(x) = \bar d(x) \gamma_5 s(x)$ and
$A_{\mu,ds}(x) = \bar d(x) \gamma_\mu \gamma_5 s(x)$. As shown in ref.~\cite{tmqcd:pap1}, once the lattice theory is renormalized in a mass independent renormalization scheme, such quantites are related, up to cutoff effects, to those of the lattice twisted theory through the quark field chiral rotations\footnote{Our notation is the following: the superscript ``cont" denotes continuum quantities, while $[ \cdots]_{\rm R}$
stands for lattice (re)normalized quantities, corresponding to either tm or OS discretization.}
\begin{equation}
\psi^{\rm cont}(x) =  \exp [ \frac{i}{2} \gamma_5 \tau^3 \alpha ] \,\, [\psi(x)]_{\rm R}
\qquad \qquad
\bar \psi_{\rm cont}(x)  =  [\bar \psi(x)]_{\rm R} \,\, \exp [ \frac{i}{2} \gamma_5 \tau^3 \alpha ] \,\, ;
\end{equation}
the phase $\alpha$ is the so-called twist-angle, defined through $\tan(\alpha) = \mu_R / m_R$.
This of course refers to the standard tmQCD formulation, with an isospin quark doublet $\psi$ and
a twisted mass term of the form $i \mu \bar \psi \gamma_5 \tau_3 \psi$. For the case under consideration,
with a distinct action~(\ref{tmQCD_action2}) for each flavour, the corresponding rotations of the valence quark fields are
\begin{equation}
f(x)^{\rm cont}  =  \exp [ \pm \frac{i}{2} \gamma_5 \alpha ] \,\, [f(x)]_{\rm R}
\qquad \qquad
\bar f(x)^{\rm cont}  =  [\bar f(x) ]_{\rm R} \,\, \exp [ \pm \frac{i}{2} \gamma_5 \alpha ] \,\, ,
\end{equation}
where the sign of the phase is that of the corresponding mass term $\mu_f$.
In order to ensure automatic improvement, we consider the case of maximal twist ($\alpha = \pm \pi/2$),
for which the above chiral rotations  induce the following relations for the two-fermion operators 
under consideration:
\begin{eqnarray}
P^{\rm cont}_{ds}  = & [P^{\rm tm}]_{\rm R}&  =  \hspace*{0.5cm} Z_P P^{\rm tm}_{ds}
\label{eq:Ptm}\\
A_{\nu,ds}^{\rm cont}  =  & \hspace{-0.25cm} - i [ V_{\nu,ds}^{\rm tm}]_{\rm R}&  =  -i Z_V  V_{\nu,ds}^{\rm tm}
\label{eq:Atm}\\
P^{\rm cont}_{ds}  =  & \hspace{-0.15cm}i [S^{\rm OS}]_{\rm R}&  =  \hspace*{0.35cm} i Z_S S^{\rm OS}_{ds}
\label{eq:POS}\\
A_{\nu,ds}^{\rm cont}  =  & [A_{\nu,ds}^{\rm OS}]_{\rm R}&  = \hspace*{0.5cm} Z_A  A_{\nu,ds}^{\rm OS} \,\, .
\label{eq:AOS}
\end{eqnarray}
All such relations are understood to be shorthand expressions for equations between correlation
functions (or matrix elements) involving these operators, valid up to discretization effects.

Maximal twist is achieved by tuning the standard mass parameter $m_0$ to its critical value $m_{\rm cr}$ (i.e. the hopping parameter is set to  $\kappa_{\rm cr}$). There are several ways of doing this. A popular procedure consists in selecting a two-point correlation function, which is trivially naught in the continuum, on account of its violating parity and flavour symmetry. At fixed $\mu$, the point $m_0 = m_{\rm cr}(\mu)$ is located, for which the correlation function vanishes. Finally, the critical mass  $m_{\rm cr}$ is found by extrapolating $m_{\rm cr}(\mu)$ to $\mu=0$ (unless the smallness of $\mu$ renders the extrapolation redundant). For details see ref.~\cite{Frezzotti:2005gi}. 
This so-called ``optimal" estimate of $m_{\rm cr}$, is characterized by the absence  of $O(a^{2k})$ discretization effects (with $k$ integer). It does however have $O(a)$ effects, while physical quantities like hadronic masses and matrix elements are automatically improved.

In the present work, we follow a very different approach, described in detail in refs.~\cite{Dimopoulos:2006dm, Dimopoulos:2007cn}. It consists in using the standard Schr\"odinger Functional estimate of $m_{\rm cr}$, by requiring the vanishing of the PCAC quark mass, as in ref.~\cite{Capitani:1998mq}. This procedure implements standard (non-twisted) Wilson fermions,  thus obtaining an explicitly $\mu$-independent estimate of $m_{\rm cr}$. However, in order for our  $m_{\rm cr}$ to be $O(a)$-improved,
both the fermionic action and the axial current in the PCAC relation must have $O(a)$  Symanzik-counterterms. Therefore the non-perturbative estimates of $c_{\rm SW}$ and $c_A$, determined with standard Wilson fermions are essential in this procedure. With $m_{\rm cr}$ thus obtained in a non-twisted, improved Wilson fermion setup, we compute hadronic masses and matrix elements in a maximally twisted framework.
This approach has also been adopted in ref.~\cite{Becirevic:2006ii}, with lattices having periodic,
rather than Schr\"odinger Functional, boundary conditions. In that work, a detailed comparison is made,
at $\beta = 6.0$, between pseudoscalar masses and decay constants (of the tm variety), obtained with the two estimates of $\kappa_{\rm cr}$ described above.

An important consequence, shared by these methods of tuning to maximal twist, is that the so-called ``infrared divergences" of the form $a/m_\pi^2$, present  in lattice correlation functions of fermion multi-local operators, are reduced to $a^2 \times a/m_\pi^2$; cf. ref.~ \cite{Frezzotti:2005gi}. This is however of little consequence to our results, obtained close to the $K$-meson  mass region, far from the chiral limit.
